Leveraging Conflicting Constraints in Solving Vehicle Routing Problems

The Conflict-Free Electric Vehicle Routing Problem (CF-EVRP) is a combinatorial optimization problem of designing routes for vehicles to visit customers such that a cost function, typically the number of vehicles or the total travelled distance, is minimized. The CF-EVRP involves constraints such as time windows on the delivery to the customers, limited operating range of the vehicles, and limited capacity on the number of vehicles that a road segment can simultaneously accommodate. In previous work, the compositional algorithm ComSat was introduced and that solves the CF-EVRP by breaking it down into sub-problems and iteratively solve them to build an overall solution. Though ComSat showed good performance in general, some problems took significant time to solve due to the high number of iterations required to find solutions that satisfy the road segments' capacity constraints. The bottleneck is the Path Changing Problem, i.e., the sub-problem of finding a new set of shortest paths to connect a subset of the customers, disregarding previously found shortest paths. This paper presents an improved version of the PathsChanger function to solve the Path Changing Problem that exploits the unsatisfiable core, i.e., information on which constraints conflict, to guide the search for feasible solutions. Experiments show faster convergence to feasible solutions compared to the previous version of PathsChanger.

==> Reviewers_comments.tex <==
Associate Editor

The paper was reviewed by two reviewers. After my own perusal, I concur with the reviewers on the suggestion that the paper can be accepted, provided that some improvements are made regarding presentation, state of the art description and positioning within it, as well as validation.

Reviewer 4

This manuscript studies the Unsatisfiable Core strategy to guide feasible solution search for vehicle routing problems with capacity constraints. The studied topic is interesting, and the paper is well structured. However, it can be improved from the following aspects.

1.	More latest relevant papers need to be introduced in Introduction for general readers. For example, ‘Integrated Task Assignment and Path Planning for Capacitated Multi-Agent Pickup and Delivery (2021)’ has designed efficient task assignment algorithms for capacitated multi-agent pickup and delivery problem, which is very relevant to the studied topic.
Sabino: DONE

2.	In Section II, the variable m is unclear, and the number of vehicles seems not given. Furthermore, it is confusing for defining&#952;p= <&#10216;n1, . . . , nm>, and m=|&#952;p|-1, where the definition of m is missing. 
Sabino: I ADDED SOME DESCRIPTIONS ABOUT THIS POINT, BUT ISN’T IT CLEAR THAT M IS JUST AN INDEX? I AM ACTUALLY THINKING ABOUT REMOVING THE ADDITIONAL LINES I INCLUDED. MOREOVER, THE WAY WE DESCRIBE THE ROUTE, THERE IS NO NEED TO TALK ABOUT VEHICLES.

3.	Some key parts in Fig. 1 are unclear. 
First, the full name of SAT is missing. 
Sabino: WORD "SAT" REMOVED

Second, the mechanism of function Router is also not clear. The manuscript presents that ‘This optimization problem is handled by the function Router and must guarantee that the routes meet specific requirements such as maximum length, specific ordering among the customers and time windows. If this step is infeasible (not SAT) then the CF-EVRP instance has no solution and the algorithm terminates.’ It is not clear how Router calculates routes that meet specific requirements such as maximum length, specific ordering among the customers and time windows. If this step is infeasible (not SAT), it is not necessary that the CF-EVRP instance has no solution as it depends on whether the function Router can search all possible routes for the problem. 
Sabino: I ADDED A REFERENCE TO THE TASE PAPER, WE CANNOT RE-EXPLAIN COMSAT FROM SCRATCH HERE

4.	Some sentences has too many ‘that’ to be understood such as ‘This has the consequence that for an infeasible problem with a MUC C, adding to the problem a constraint that rules out that all the constraints in C are simultaneously active will resolve that particular conflict’. 
MF: I edited this sentence slightly.

5.	Section V can be improved. First, more simulation results are needed for the comparisons of PC and GPC such as comparing their performance for optimizing the objective function instead of only comparing the running time.
Sabino: WE DECIDED NOT TO RUN FURTHER SIMULATIONS

Second, it seems that GPC is better than PC in instance 5 shown in Table I, which is not the case as analyzed. 
Sabino: EHM....I DON'T KNOW WHAT HE/SHE IS TALKING ABOUT, THIS IS NOT WHAT IT SAYS IN TABLE I

Third, please mark clearly whether the time shown in Table I is the running time of the strategy in each iteration or it is the overall execution time. 
Sabino: I ADDED THE WORD "TOTAL" IN THE TABLE CAPTION 


Reviewer 8 

The authors propose a good extension of their previous work, that fixes one of the main issues found during the experimental campaign. The quality of the article is quite good, anyway, I will suggest some improvements (listed below) to enhance the overall work:

- For the ones who are not into the topic it is difficult to understand from the title what is the main subject of the article. Try to use a more attractive one.
Sabino: MAYBE HE HAS A POINT...I HAVE BEEN THINKING ABOUT ANOTHER TITLE...ANY SUGGESTION?
%% Current title:
%% Using the Unsatisfiable Core to Guide Feasible Solution Search for Vehicle Routing Problems with Capacity Constraints
MF: Using Knowledge of Conflicting Constraints to Guide Feasability Search in Vehicle Routing Problems
MF: Using Knowledge of Conflicting Constraints to Improve the Solution Times for Vehicle Routing Problems
MF: Leveraging Conflicting Constraints to Speed Up Feasible Solution Search in Vehicle Routing Problems
MF: Improving the Feasible Solution Search in Vehicle Routing Problems by Using Knowledge of Conflicting Constraints.

% - The introduction is lacking of information related to the state of the art and the position of your work concerning the one already published in the literature. 
Sabino: DONE
% - I would like to see some more experiments and comparisons % with the two methods to enhance the improvements gained % with the new implementation.
Sabino: WE DECIDED NOT TO RUN FURTHER SIMULATIONS

The rest of the article is consistent and well structured, I suggest accepting it to the conference.

==> experiments.tex <==
\section{Computational Analysis} \label{experiments}

In order to compare \MonoMod and \theAlgorithm we generated a set of problem instances. The parameters we used are the number of nodes, vehicles, and jobs (grouped in an index called N-J-V), as well as the time horizon and the value called 'edge reduction', which indicates the connectivity of the graph (the higher the value, the fewer edges). For each combination of these parameters, five different problems are randomly generated.

For the analysis we used Z3 4.8.9. The time limit for \MonoMod is set to 10800 seconds (three hours); the model generation time is measured separately, since it is implementation-dependent and can be dealt with using more efficient formulations, as discussed in our previous work \cite{roselli2020compact}. As for \theAlgorithm, we only computed \emph{ten} paths for each pair of customers. We also set an upper bound of \emph{ten} to the number of iterations between the \emph{Routing Problem} and the \emph{Assignment Problem}. Also, the generation time refers to the time taken to generate the paths between each pair of customers. All the experiments were performed on an \emph{Intel Core i7 6700K, 4.0 GHZ, 32GB RAM}  running \emph{Ubuntu-18.04 LTS}.

Though Z3 allows for optimization of the objective function, the size of the problems evaluated with \MonoMod is such that no optimum is expected to be found in any reasonable time. Therefore Z3 is set to find feasible, sub-optimal solutions \footnotemark.

Table~\ref{tab:table_I} summarizes the results of the computational analysis. The generation time for \theAlgorithm is actually negligible, whereas for \MonoMod it increases with N-J-V (nodes, vehicles, and jobs), and time horizon and it decreases with the \emph{edge reduction}, presumably because fewer edges means fewer constraints to declare. By comparing the number of solved instances in each category, whether they turned out to be \emph{sat} or \emph{unsat}, it is possible to notice that there is a number of instances that were determined \emph{unknown} by \theAlgorithm but were declared \emph{unsat} by \MonoMod. On the other hand, both methods usually agree on the feasibility of the \emph{sat} instances, except for some cases with high values of N-J-V and time horizon where \MonoMod run out of time. The reason for the \emph{unknown} responses lies in the termination criterion we set up for the algorithm. By running early experiments we noticed that the algorithm was rather slow in evaluating unsatisfiable problem instances; therefore we decided to limit the number of iterations between the \emph{Routing Problem} and the \emph{Assignment Problem}. On average, \theAlgorithm is between 10 and 100 times faster than the  at solving instances that are intrinsically \emph{sat}.
% When it comes to the running time, the compositional algorithm is faster than the monolithic model and the gap between them increases with the problem complexity (in terms of N-J-V and time horizon). The plot in Figure~\ref{fig:methods} provides a graphical representation of the performance of the two approaches by showing the ratio between the solving time of the compositional algorithm and the monolithic model. Each dot represents an instance, and if the dot is above the blue line it means that the monolithic model was faster to solve that instance than the compositional algorithm; if the dot is below the line the compositional algorithm was faster. The blue dots above the line represent the instances that were declared \emph{unknown} by the compositional algorithm but not by monolithic model; the blue dots below the blue line represent the instances that could were declared \emph{unknown} by the monolithic model but not by the compositional algorithm. To plot this graph, instances have been sorted by N-J-V, time horizon, and edge reduction respectively. 
